Meta Learning with Differentiable Closed-form Solver for Fast Video Object Segmentation

This paper tackles the problem of video object segmentation. We are specifically concerned with the task of segmenting all pixels of a target object in all frames, given the annotation mask in the first frame. Even when such annotation is available this remains a challenging problem because of the changing appearance and shape of the object over time. In this paper, we tackle this task by formulating it as a meta-learning problem, where the base learner grasping the semantic scene understanding for a general type of objects, and the meta learner quickly adapting the appearance of the target object with a few examples. Our proposed meta-learning method uses a closed form optimizer, the so-called "ridge regression", which has been shown to be conducive for fast and better training convergence. Moreover, we propose a mechanism, named "block splitting", to further speed up the training process as well as to reduce the number of learning parameters. In comparison with the-state-of-the art methods, our proposed framework achieves significant boost up in processing speed, while having very competitive performance compared to the best performing methods on the widely used datasets.

==> figs/J_F2016.tex <==
\begin{table*}[ht]
\begin{center}
\scalebox{0.9}{
{\begin{tabular}{l c| c c c c c c c c c c c c c c} 

\hline
Measure &    & OSVOS & MLV(ours) & MSK & PML & SFL  & CTN & VPN & OFL & BVS & FCP & JMP & HVS &  SEA\\ 

\hline
J\&F   &  Mean  & 80.2  & x & 77.5 & 77.4 & 76.0 & 71.4 & 67.8 & 65.7 & 59.4 & 53.8 &  55.1 & 53.8 & 49.2 \\ 

\hline
& Mean & 79.8 & 75.5 &  79.7 & 75.5 & 76.1 & 73.5 & 70.2 & 68.0 & 60.0 & 58.4 & 57.0 & 54.6 & 50.4\\ %& 

J & Recall & 93.6 & x & 93.1 & 89.6 & 90.6 &  87.4 &  82.3 & 75.6 & 66.9 & 71.5 &  62.6 & 61.4 & 53.1 \\

 & Decay & 14.9 & x & 8.9 & 8.5 & 12.1 & 15.6 & 12.4 & 26.4 & 28.9 & -2.0 & 39.4 & 23.6 &  36.4\\

\hline
& Mean & 80.6 & y & 75.4 & 79.3 & 76.0 & 69.3 & 65.5 & 63.4 & 58.8 & 49.2 & 53.1 & 52.9 & 48.0\\

F & Recall & 92.6 & y & 87.1 & 93.4 & 85.5 & 79.6 & 69.0 & 70.4 & 67.9 & 49.5 & 54.2 & 61.0 & 46.3 \\

   & Decay & 15.0 & y & 9.0 & 7.8 & 10.4 & 12.9 & 14.4 & 27.2 & 21.3 & -1.1 &   38.4 & 22.7 & 34.5\\ 
\hline   
T & Mean & 37.8 & z & 21.8 & 47.0 & 18.9 & 22.0 & 32.4 & 22.2 & 34.7 & 30.6 & 15.9 & 36.0 & 15.4 \\ 
\hline

\end{tabular}
}

\label
{tab:QuantitativeResults}}
\caption{Evaluation results on Davis 2016 validation set: A comprehensive comparison with the rent state-of-the-art methods}

\end{center}
\end{table*}

==> figs/addson_2017.tex <==

\begin{table*}[t]
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|}
\hline
Method & Online-Tuning & J mean & J recall & J Decay & F mean & F recall & F Decay \\

\hline
OSVOS-B & \xmark & 18.5 & 15.9 & -0.8 & 30.0 & 20.0 & 0.1 \\

\hline
MaskTrack-B & \xmark & 35.3 & 37.8 & 39.3 & 36.4 & 36.0 & 42.0 \\

\hline
OSVOS-M & \xmark & 36.4 & 34.8 & 14.8 & 39.5 & 35.3 & 9.1 \\

\hline
MaskTrack-M & \xmark & 44.6 & 48.7 & 27.1 & 47.6 & 49.3 & 27.9 \\

\hline
OSVOS & \cmark & 55.1 & 60.2 & 28.2 &  62.1 & 71.3 & 29.3 \\

\hline
MaskTrack & \cmark & 51.2 & 59.7 & 28.3 & 57.3 & 65.5 & 29.1 \\
\hline

OSNM & \xmark & 52.5 & 60.9 & 21.5 & 57.1 & 66.1 & 24.3\\
\hline

Ours & \xmark & \textcolor{red}{x} & \textcolor{red}{x} & \textcolor{red}{x} & \textcolor{red}{x} & \textcolor{red}{x} & \textcolor{red}{x} \\
\hline

\end{tabular}
\end{center}
\caption{Adds on results on Davis2017}
\end{table*}
